Pre-training Generative Recommender with Multi-Identifier Item Tokenization

Generative recommendation autoregressively generates item identifiers to recommend potential items. Existing methods typically adopt a one-to-one mapping strategy, where each item is represented by a single identifier. However, this scheme poses issues, such as suboptimal semantic modeling for low-frequency items and limited diversity in token sequence data. To overcome these limitations, we propose MTGRec, which leverages Multi-identifier item Tokenization to augment token sequence data for Generative Recommender pre-training. Our approach involves two key innovations: multi-identifier item tokenization and curriculum recommender pre-training. For multi-identifier item tokenization, we leverage the RQ-VAE as the tokenizer backbone and treat model checkpoints from adjacent training epochs as semantically relevant tokenizers. This allows each item to be associated with multiple identifiers, enabling a single user interaction sequence to be converted into several token sequences as different data groups. For curriculum recommender pre-training, we introduce a curriculum learning scheme guided by data influence estimation, dynamically adjusting the sampling probability of each data group during recommender pre-training. After pre-training, we fine-tune the model using a single tokenizer to ensure accurate item identification for recommendation. Extensive experiments on three public benchmark datasets demonstrate that MTGRec significantly outperforms both traditional and generative recommendation baselines in terms of effectiveness and scalability.

==> sec2_preliminary.tex <==
\section{Preliminary}
\label{sec:preliminary}
Given the item set $\mathcal{V}$, let $S = [v_1, v_2, \dots, v_t]$ denote the user's historical interacted items in chronological order.
Sequential recommendation aims to capture user preferences implicit in the item sequence and predict the next potential item $v_{t+1}$.
Generative recommendation reformulates the traditional sequential recommendation task as a sequence-to-sequence problem. 
In this paradigm, the prediction is achieved by autoregressively generating the identifier of the target item, which is represented as a token sequence.
Specifically, a typical generative recommender system involves two crucial components~\cite{tiger,letter}: (i) an \emph{item tokenizer} for mapping each item to its corresponding identifier
and (ii) a \emph{generative recommender} for autoregressive generation.
Below, we elaborate on the details of these two crucial components. 






\subsection{Item Tokenizer}
\label{sec:item_tokenizer}
To begin with, an item tokenizer is learned to associate each item with a series of tokens that imply semantic knowledge. 
Formally, we denote the item tokenization as $[c_1,\dots,c_H] = \mathrm{T}(v)$, where $c_h$ represents the $h$-th token of $v$, $H$ is the length of the identifier and $\mathrm{T}$ denotes the item tokenizer.
In practice, the predominant item tokenizer utilized in generative recommendation is RQ-VAE~\cite{rqvae}, which is advantageous due to its efficacy in modeling prior semantics and mitigating length bias~\cite{letter,seater}.
Initially, RQ-VAE takes the item semantic embedding $\bm{z}$ (\eg text embedding encoded by a pre-trained language model) as input and encodes it into a latent representation $\bm{r}$.
Then, $\bm{r}$ is quantized into serialized codes~(called tokens) from coarse to fine by looking up $H$-level codebooks. 
Each level's codebook is denoted by $\mathcal{C}^h = \{\bm{e}_k^h\}_{k=1}^K$, where $\bm{e}_k^h$ is a learnable cluster center and $K$ is the codebook size. 
Finally, the residual quantization is applied to $\bm{r}$:
\begin{align}
    & c_h = \underset {k} { \operatorname {arg\,min} } ||\bm{r}_h - \bm{e}_k^h||_2^2, \\
    & \bm{r}_{h+1} = \bm{r}_h - \bm{e}_{c_h}^h,
    \label{eq:rq}
\end{align}
where $\bm{r}_h$ is the residual vector in the $h$-th RQ level, and $\bm{r}_1 = \bm{r}$. 
Thereafter, we obtain the item quantized representation $\tilde{\bm{r}}=\sum_{h=1}^H\bm{e}^h_{c_h}$ and feed it into a decoder to reconstruct the item semantic embedding.
Overall, the optimization objectives of the item tokenizer are as follows:
\begin{align}
    \mathcal{L}_{\mathrm{T}} & = \mathcal{L}_{\text{recon}} + \mathcal{L}_{\text{rq}},  \\
    \mathcal{L}_{\text{recon}} &= ||\bm{z} - \hat{\bm{z}}||_2^2, \\
    \mathcal{L}_{\text{rq}} &= \sum_{h=1}^{H} ||\operatorname{sg}[\bm{r}_h] - \bm{e}_{c_h}^h||_2^2 + \beta \ ||\bm{r}_h - \operatorname{sg}[\bm{e}_{c_h}^h]||_2^2, 
    \label{eq:rqloss}
\end{align}
where $\hat{\bm{z}}$ is the reconstructed item embedding, and $\operatorname{sg}[\cdot]$ denotes the stop-gradient operation. 
$\beta$ is the coefficient to balance the optimization between the encoder and codebooks, typically set to 0.25.













\subsection{Generative Recommender}
Based on the learned item tokenizer, the interacted item sequence $S$ and the target item $v_{t+1}$ are tokenized into token sequences, denoted as $X = \mathrm{T}(S) = [c^1_1,c^1_2, \dots, c^t_{H-1},c^t_H]$  and $Y = \mathrm{T}(v_{t+1}) = [c^{t+1}_1,\dots,c^{t+1}_H]$ respectively.
Following this, the token sequence $X$ is fed into a generative model (\eg T5~\cite{t5}) to generate $Y$ in an autoregressive manner:
\begin{align}
    P(Y|X) = \prod_{h=1}^H  P(c^{t+1}_h|X,c^{t+1}_1,\dots,c^{t+1}_{h-1}).
\end{align}
As for model optimization, we leverage the negative log-likelihood of the target token sequence $Y$ as the loss for the generative recommender, which can be written as:
\begin{align}
    \mathcal{L}(X,Y) = - \sum_{h=1}^{H}\operatorname{log} P(c^{t+1}_h|X,c^{t+1}_1,\dots,c^{t+1}_{h-1}).
    \label{eq:lmloss}
\end{align}
Regarding inference, generative recommendation methods usually adopt beam search to decode $N$ token sequences and map them to corresponding items for top-$N$ recommendation.



% \begin{align}
%    & \mathrm{T} \sim \{\mathrm{T}_1, \mathrm{T}_2, \dots, \mathrm{T}_n\} \\
%    \text{where} \quad &  P(\mathrm{T}_i)= p_i, \quad \sum_{i=1}^n p_i = 1
% \end{align}

% \begin{align}
%    X &= \mathrm{T}(S) = [c^1_1,c^1_2, \dots, c^t_{H-1},c^t_H] \\
%    Y &= \mathrm{T}(v_{t+1}) = [c^{t+1}_1,\dots,c^{t+1}_H]
% \end{align}

% \begin{align}
%     \mathcal{L} = - \sum_{j=1}^{H}\operatorname{log} P(c^{t+1}_j|X,c^{t+1}_1,\dots,c^{t+1}_{j-1})
% \end{align}

% \begin{align}
%     \mathcal{L} = - \sum_{j=1}^{H}\operatorname{log} P(c^{t+1}_j|X,c^{t+1}_1,\dots,c^{t+1}_{j-1})
% \end{align}


% \begin{align}
%     \mathcal{L}(\mathcal{D}_{val};\bm{\theta}^{t+1}) = \mathcal{L}(\mathcal{D}_{val};\bm{\theta}^{t}) + \nabla \mathcal{L}(\mathcal{D}_{val};\bm{\theta}^{t}) \cdot (\bm{\theta}^{t+1} - \bm{\theta}^{t})
% \end{align}


% \begin{gather}
%     \bm{\theta}^{t+1}-\bm{\theta}^{t} = -\eta_{t} \Gamma\left(\mathcal{D}_{train}, \bm{\theta}^{t}\right) \\
%     \Gamma\left(\mathcal{D}_{train}, \bm{\theta}^{t}\right) = \frac{\bm{m}^{t+1}}{\sqrt{\bm{v}^{t+1}+\epsilon}} \\
% \bm{m}^{t+1}  =\left(\beta_{1} \bm{m}^{t}+\left(1-\beta_{1}\right) \nabla \mathcal{L}\left(\mathcal{D}_{train}; \bm{\theta}^{t}\right)\right) /\left(1-\beta_{1}^{t}\right) \\
% \bm{v}^{t+1} =\left(\beta_{2} \bm{v}^{t}+\left(1-\beta_{2}\right) \nabla \mathcal{L}\left(\mathcal{D}_{train}; \bm{\theta}^{t}\right)^{2}\right) /\left(1-\beta_{2}^{t}\right)
% \end{gather}

% \begin{align}
%     \text{Inf}(\mathrm{T}_i) = \sum_{k=1}^{K} \eta_{k} \nabla \mathcal{L}\left(\mathcal{D}_{val} ; \bm{\theta}_{k}\right) \cdot \Gamma\left(\mathcal{D}_{train}^i, \bm{\theta}_{k}\right)
% \end{align}

% \begin{align}
%     p_i =  \frac{e^{ \text{Inf}(\mathrm{T}_i) / \tau} }{\sum_{j=1}^n e^{\text{Inf}(\mathrm{T}_j) / \tau} }
% \end{align}


% \begin{align}
%     & c_j = \underset {k} { \operatorname {arg\,min} } ||\bm{r}_j - \bm{e}_k^j||_2^2 \\
%     & \bm{r}_{j+1} = \bm{r}_j - \bm{e}_{c_j}^j
%     \label{eq:rq}
% \end{align}

% \begin{align}
%     \mathcal{L}_{\mathrm{T}} & = \mathcal{L}_{\text{recon}} + \mathcal{L}_{\text{rq}}  \\
%     \mathcal{L}_{\text{recon}} &= ||\bm{z} - \hat{\bm{z}}||_2^2 \\
%     \mathcal{L}_{\text{rq}} &= \sum_{j=1}^{H} ||\operatorname{sg}[\bm{r}_j] - \bm{e}_{c_j}^j||_2^2 + \beta \ ||\bm{r}_j - \operatorname{sg}[\bm{e}_{c_j}^j]||_2^2
%     \label{eq:rqloss}
% \end{align}
